Preserving Stabilization while Practically Bounding State Space

Stabilization is a key dependability property for dealing with unanticipated transient faults, as it guarantees that even in the presence of such faults, the system will recover to states where it satisfies its specification. One of the desirable attributes of stabilization is the use of bounded space for each variable. In this paper, we present an algorithm that transforms a stabilizing program that uses variables with unbounded domain into a stabilizing program that uses bounded variables and (practically bounded) physical time. While non-stabilizing programs (that do not handle transient faults) can deal with unbounded variables by assigning large enough but bounded space, stabilizing programs that need to deal with arbitrary transient faults cannot do the same since a transient fault may corrupt the variable to its maximum value. We show that our transformation algorithm is applicable to several problems including logical clocks, vector clocks, mutual exclusion, leader election, diffusing computations, Paxos based consensus, and so on. Moreover, our approach can also be used to bound counters used in an earlier work by Katz and Perry for adding stabilization to a non-stabilizing program. By combining our algorithm with that earlier work by Katz and Perry, it would be possible to provide stabilization for a rich class of problems, by assigning large enough but bounded space for variables.

==> algorithm.tex <==
\iffalse
\section{Algorithm}
\subsection{Problem specification}

%m bound example
%%Figure 
\begin{figure}
  \hfill\includegraphics[width=70mm, scale=1.0]{figures/m_bounded_intervals.jpg}\hspace*{\fill}
  \caption{Range of counter $x$}
  \label{fig:m_bounded_intervals}
\end{figure}

In this section, we present our algorithm for transformation of a program with free and dependent counters into a stabilizing program that uses one unbounded variable that identifies the physical time of the process and a set of bounded variables. 

%As mentioned in the Introduction, our goal is to utilize an unbounded variable that represents the current time and requiring that all other variables be bounded. 

%This is a test to see how good the program works with concurrent updates


%\newcommand{\regionsize}{SZ\xspace}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
We proceed as follows: let $t.j$ denote the time  associated with process $j$.  First, we partition  time into multiple regions of equal size, say $w$.
The region of $j$, denoted by $R.j$, is %$\floor{\frac{t.j}{\regionsize}}$. 
$\floor{\frac{t.j}{w}}$. 
We choose $w$ to be such that any two processes differ by at most one region. In other words, 
$\text{for any two processes, }$ $j$ and $k$, $|R.j - R.k| \leq 1$.  Clearly, this is possible with modern systems with use of services such as NTP. For example, if we choose $w$ to consist of an hour, it is clearly possible to ensure that clock of two processes do not differ by more than an hour. 

Next, our goal is to ensure that the values of all variables whose domain is the set of natural numbers can be changed to that where their new domain is finite. We will achieve this by relating the value of the variable to the current region that $j$ finds itself in. BUT THIS DOES NOT MAKE THE DOMAIN FINITE RIGHT ? V does right? 

%-- Added above. 

Each process has a counter $x$ associated with it. For a process $j$ the value of $x.j$ at any point in time is linked with the current region i.e. value of $R.j$. 
When $R.j$ increases i.e.when the process $j$ moves to the next region, any counter associated with that process should have progressed to the new region.

\iffalse
%bound on x using v

\iffalse
So as shown in figure \ref{fig:m_bounded_intervals}, if the counter $x$ is associated with the last region i.e. region $m$, an increase in the value of $x$ can preserve the association of $x$ to the $m^{th}$ region or can now be linked with region $1$, i.e. regions restart after $m$. 

At any point in time the value of $x$ is in one of the $m$ intervals, so 
For example if $x$ is in interval $i$ then the value of $x$ is in the range $\{(i-1)w,iw\}$, after $x=iw$ upon executing the next increment operation on $x$, the value of the counter moves to the next interval $i+1$. 
\fi

The requirements of the system are as follows:

(i)The counters of the processes increment their values and never decrement,

(ii)The counters of any two processes are at most $1$ region apart from each other.

\iffalse
\subsection{Fault Span}
For a process $j$, if $R.j$ is the variable that denotes the interval in which the counter $x.j$ lies, then the fault span $FS$ that has to be preserved at all times by both program actions and fault actions in this asynchronous system can be denoted as,

$\text{For any process } k \neq j, |R.j - R.k| \leq 1$

//text about how R is updated?
\fi

\subsection{Invariant}
Now we define the invariant $S$ that consists of the set of constraints that are always true in the given program in the absence of faults. If these set of constraints hold in the initial state of program i.e. if the program starts its execution within the invariant then in the absence of faults the program continues to stay in the invariant, i.e. the set of constraints continue to hold. On encountering a fault the program may not satisfy the set of constraints. But once the faults stop and when the program recovers back to the invariant by performing the required repair actions, then it is guaranteed to stay within the invariant in the absence of faults.

We introduce two variables $h,l$, such that 

\indent\indent$h = max\{R.j\ |\text{ j is a process in the given asynchronous system}\}$,

\indent\indent$l = min\{R.j\ |\text{ j is a process in the given asynchronous system}\}$.

In other words $h,l$ are the highest and the lowest regions that contain some process-counter $x.j$ (of process $j$).

%%Figure 
\begin{figure}
\centering
	\begin{subfigure}{.5\textwidth}
	\centering
	\includegraphics[width=.6\linewidth]{figures/Counter_with_respect_to_h.jpg}
	\caption{}
	\end{subfigure}%	
	\begin{subfigure}{.5\textwidth}
	\centering
	\includegraphics[width=.6\linewidth]{figures/Counter_with_respect_to_l.jpg}
	\caption{}
	\end{subfigure}
	
\caption{Allowed range of value of counter with respect to $h,l$}
\label{fig:Counter_with_respect_to_l_h}
\end{figure}


%As per the fault span $FS: |R.j - R.k| \leq 1$, so to ensure this 
The first constraint $S1$ in the invariant $S$ is,

\indent\indent\indent\indent\indent$S1: \forall j: \{x.j \in \{(h-1)w \cdots (h+1)w\}\} \vee \{x.j \in \{(l-1)w \cdots (l+1)w\}\}$

As shown in figures \ref{fig:Counter_with_respect_to_l_h} (a) and (b), the value of any counter in the program can be one region ahead of $l$ or $h$.This is ensured by $S1$.
%, since the difference between the regions of any two process-counters is at most $1$. This is ensured by $S1$. 
Observe that when $l==h$ figures \ref{fig:Counter_with_respect_to_l_h} (a) and (b) refer to the same regions. 

%However, if a counter $x.j$ of process $j$ is in the region $h-1$ then a counter $x.k$ of process $k \neq j$ is not allowed to be in region $h+1$, because in this case the counters are two regions apart and thereby violate the second requirement of the system. Similarly, if a counter $x.j$ of process $j$ is in the region $l-1$ then a counter $x.k$ of process $k \neq j$ is not allowed to be in region $l+1$. So if $l==h$, then the following constraint $S2$ will handle both of these scenarios,

%$S2: \forall k \neq j: \{x.j \in \{(l-2)w \cdots (l-1)w\} \implies \not \exists x.k \in \{lw \cdots (l+1)w\}\}$

%$S3: \forall k \neq j: \{x.j \in \{(h-2)w \cdots (h-1)w\} \implies \not \exists x.k \in \{hw \cdots (h+1)w\}\}$

%m bound example
%%Figure 
\begin{figure}
  \hfill\includegraphics[width=50mm, scale=1.0]{figures/Counter_with_respect_to_l_h_when_different.jpg}\hspace*{\fill}
  \caption{Determining legal intervals when $l \neq h$}
  \label{fig:Counter_with_respect_to_l_h_when_different}
\end{figure}


%If $l==h$, $S= S1 \wedge S2 \wedge S3$ ensure convergence to the fault span.
%If $l==h$, $S= S1 \wedge S2$ ensure convergence to the fault span.
However when $l \neq h$, $l,h$ are one region apart as shown in figure \ref{fig:Counter_with_respect_to_l_h_when_different}. In this case, if a counter $x.j$ of process $j$ is in the region $l$ then a counter $x.k$ of process $k \neq j$ is not allowed to be in regions $h+1$, because in this case the counters are two or regions apart. 
%Similarly, the counters can violate the region requirement the other direction i.e.if a counter $x.j$ of process $j$ is in the region $h+1$ then a counter $x.k$ of process $k \neq j$ is not allowed to be in region $l$. 
So we add the following constraint $S2$ to the invariant,

\indent\indent\indent\indent\indent$S2: \forall j: \{ \forall k \neq j: \{\{x.j \in \{(l-1)w \cdots lw\}\} \wedge \{l \neq h\}\} \implies \{\not \exists x.k > hw\}\}\}$

%$S4: \forall k \neq j: \{\{x.j \in \{hw \cdots (h+1)w\}\} \wedge \{l \neq h\}\} \implies \{\not \exists x.k < lw\}\}$

\noindent So combining the constraints, the invariant          

\indent\indent\indent\indent\indent\indent\indent$S = S1 \wedge S2$.

\subsection{Standard Actions}
Now we will define the set of actions that the processes perform in the absence of faults, i.e. when the program is within the invariant.

1. A process can increment its counter by some positive constant $a$. 

\indent\indent\indent\indent\indent\indent\indent$true \Rightarrow \{a \geq 0 \wedge x.j = x.j + a\}$



2. $R$ value of each process is updated periodically by some reliable service like NTP. So whenever the $R$ value is updated the following action is executed, 

$(R.j > old\_R.j) \rightarrow \{\neg\{([R.j]-1)*w \leq x.j \leq R.j*w\} \rightarrow \{x.j := (R.j-1)*w\}\} \wedge \{old\_R.j := R.j\}$

When R.j increases i.e.when process $j$ moves to the next region, the process checks if the value of its counter $x.j$ is within the new region and if it is outside the new region, then it is updated to the minimum value in the range of the new region. Variable $old\_R.j$ keeps track of the region in which the process $j$ is in. So the condition (guard) $R.j > old\_R.j$ ensures that whenever the process moves to the next region this action is triggered.

\textbf{Invariant closure}.
When the program is within the invariant, in the absence of faults,  if the program executes any standard actions it continues to stay within the invariant.

\textbf{Proof.}
For the sake of simplicity we consider a system of two processes $j,k$.
If the program is in a state where the two constraints $S1,S2$ hold, then 
1. On executing the first action $true \Rightarrow \{a \geq 0 \wedge x.j = x.j + a\}$ the value of the counter $x.j$ increases. 

%%Figure 
\begin{figure}
  \hfill\includegraphics[width=40mm, scale=1.0]{figures/legal_centre_l_h_equal.jpg}\hspace*{\fill}
  \caption{Case 1: $l == h$}
  \label{fig:legal_centre_l_h_equal}
\end{figure}

\begin{figure}
  \hfill\includegraphics[width=40mm, scale=1.0]{figures/legal_centre_l_h_different.jpg}\hspace*{\fill}
  \caption{Case 2: $l \neq h$}
  \label{fig:legal_centre_l_h_different}
\end{figure}

\textbf{Case 1}: Consider the scenario shown in Figure \ref{fig:legal_centre_l_h_equal} where $l == h$, with processes $j,k$ in the same region $R.j=R.k$, and their counters $x.j,x.k$ are also in the same region. Now an increase in the value of one of the counters say $x.k$, results in it moving to the next region $R.k + 1$ or in staying in the current region $R.k$. If the counter stays in the same region then it is in region $l$ or $h$, and if it moves to the next region, then it is in region $l+1$ or $h+1$, so constraint $S1$ clearly holds. Constraint $S2$ holds trivially since $l==h$ in this scenario.

\textbf{Case 2}: Consider the scenario shown in figure \ref{fig:legal_centre_l_h_different} where $l \neq h$, with processes $j,k$ in the adjacent regions $R.k=R.j+1$, and their counters $x.j,x.k$ are in the corresponding regions $Rj$ and $R.k$ respectively. Here if action $1$ is executed on $x.j$, it stays in the same region $l$ or moves to the next region $l+1$ or $h$, so constraint $S1$ clearly holds. In this scenario constraint $S2$ holds trivially since no counter is in the range $\{(l-1)w \cdots lw\}$ i.e. in region $l$ after $x.j$ moves to the next region.

\textbf{Case 3}: Consider the scenario shown in figure \ref{fig:legal_centre_l_h_different}. Here if action $1$ is executed on $x.k$, it stays in the same region $h$ or moves to the next region $h+1$, so constraint $S1$ still holds. But, constraint $S2$ does not hold momentarily since counters $x.j$ and $x.k$ are now two regions apart. However, since each process executes action $2$ periodically, after finite time when $R.j$ increases and becomes $R.j==R.k$, by executing action $2$ the counter $x.j$ is reset to the minimum value in the subsequent region, thereby reducing the gap between the two counters to one region. So constraint $S2$ also holds.

\vspace{3mm}

%Executing action $2$
If the program is in a state where the two constraints $S1,S2$ hold, then 
1. On executing the second action $(R.j > old\_R.j) \rightarrow \{\neg\{([R.j]-1)*w \leq x.j \leq R.j*w\} \rightarrow \{x.j := (R.j-1)*w\}\} \wedge \{old\_R.j := R.j\}$, i.e. when a process moves to the next region the value of the corresponding process counter is checked such that it is within the new region and if is not in the new region it is reset accordingly. 

\textbf{Case 1.}
Consider the scenario shown in figure \ref{fig:legal_centre_l_h_equal} where $l == h$, with processes $j,k$ in the same region $R.j=R.k$, and their counters $x.j,x.k$ are also in the same region. Now when one of the processes say process $j$ moves to the next region, and if $x.j$ is not already in the new region, $j$  resets the value of $x.j$ to the minimum value in the new region i.e.$(R.j-1)*w$. This new region is now $l+1$ or $h$, so constraint $S1$ continues to hold. And constraint $S2$ also holds since $x.j$ and $x.k$ are only one region apart.

\textbf{Case 2}: Consider the scenario shown in figure \ref{fig:legal_centre_l_h_different} where $l \neq h$, with processes $j,k$ in the adjacent regions $R.k=R.j+1$, and their counters $x.j,x.k$ are in the corresponding regions $Rj$ and $R.k$ respectively. Here if action $2$ is enabled at process $j$, i.e. if $j$ moves to the next region, and resets $x,j$ accordingly, $l$ and $h$ are now equal, so constraint $S1$ clearly holds. In this scenario constraint $S2$ holds trivially since $l==h$ after $j$ moves to the next region.

\textbf{Case 3}: Consider the same scenario shown in figure \ref{fig:legal_centre_l_h_different}. Here if action $2$ is enabled for $k$, it moves to the next region $h+1$, and resets $x.k$ accordingly, so constraint $S1$ still holds. 
When $R.k$ increases $R.j$ also increases since for any two processes $j,k$, $|R.j-R.k|$ has to be $\leq 1$ and $|R.j-R.k| == 1$ even before the execution of this action. So when $R.j,R.k$ increase, counters $x.j,x.k$ are also reset accordingly, such that they continue to be one region apart.
So constraint $S2$ also holds.

%fault detection and repair
\subsection{Repair Actions}

%%the only repair action required would be $\neg\{([R.j]-1)*w \leq x.j \leq R.j*w\} \rightarrow \{x.j := (R.j-1)*w\}\}$ in case of a fault

When $S1$ does not hold at a process $j$, i.e. if $x.j$ is not in the range of values defined by $S1$ we require the following action:

\indent\indent\indent\indent$r1: \{x.j \leq (l-2)w \implies x.j := (l-2)w + 1\}$

\indent\indent\indent\indent$r2: \{x.j > (h+1)w \implies x.j := hw + 1\}$

\vspace{2mm}
\indent\indent\indent\indent\indent\indent\indent\indent$R1: \neg S1 \rightarrow r1 \wedge r2$

Consider a fault at process $j$ that causes the value of counter $x.j$ at $j$ to be stuck momentarily. Convergence is possible only if faults are guaranteed to stop eventually. So after the fault the counter continues to execute its normal action. However, now it has a value less than the allowed minimum of $(l-2)w + 1$, so to converge $x.j$ is assigned the minimum value. Similarly, if a fault corrupts $x.j$ and if its value becomes more than the maximum allowed value of $(h+1)w$, then we ensure convergence by assigning $x.j$ to $hw+1$. 
Observe that we do not assign it to the maximum allowed value of $(h+1)w$. This is because a counter increment action that immediately follows such an assignment will again cause $S1$ to be violated immediately.

Next, we provide similar repair actions for violations corresponding to each of the remaining constraints in the invariant, i.e. if one of $S2,S3,S4$ do not hold.

\indent\indent\indent\indent\indent\indent\indent$R2: \neg S2 \vee \neg S3 \rightarrow x.j := (l-1)w + 1$

%\vspace{2mm}
%\indent\indent\indent\indent\indent\indent\indent$R3: \neg S3 \rightarrow x.j := (h-1)w + 1$

\vspace{2mm}
\indent\indent\indent\indent\indent\indent\indent$R3: \neg S4 \rightarrow x.j := lw + 1$

Note that $R2$ provides the corrective action for violation of both $S2$ and $S3$.
\fi
\fi
